VLP: A Survey on Vision-Language Pre-training

In the past few years, the emergence of pre-training models has brought uni-modal fields such as computer vision (CV) and natural language processing (NLP) to a new era. Substantial works have shown they are beneficial for downstream uni-modal tasks and avoid training a new model from scratch. So can such pre-trained models be applied to multi-modal tasks? Researchers have explored this problem and made significant progress. This paper surveys recent advances and new frontiers in vision-language pre-training (VLP), including image-text and video-text pre-training. To give readers a better overall grasp of VLP, we first review its recent advances from five aspects: feature extraction, model architecture, pre-training objectives, pre-training datasets, and downstream tasks. Then, we summarize the specific VLP models in detail. Finally, we discuss the new frontiers in VLP. To the best of our knowledge, this is the first survey focused on VLP. We hope that this survey can shed light on future research in the VLP field.

==> mir-sample-bib.tex <==
\begin{thebibliography}{9}



\bibitem{bib1} B. Ran, D. E. Boyce. {\sl Modeling Dynamic Transportation Network}, Berlin, Germany: Springer-Verlag, pp. 69-83,1996. (Book style)

\bibitem{bib2} G. O. Young. Synthetic structure of industrial plastics. Plastics, 2nd ed., J. Peters, Ed., New York, USA: McGraw-Hill, pp. 15-64, 1964. (Book style with paper title and editor)

\bibitem{bib3} L. C. Su, F. Zhu. Design of a novel omnidrectional stereo vision system. {\sl Acta Automatica Sinica}, vol. 32, no. 1, pp. 67-72, 2006. (in Chinese) (Periodical style)

\bibitem{bib4} R. Roychoudhury, S. Bandyopadhyay, K. Paul. Adistributed mechanism for topology discovery in ad hoc wireless networks using mobile agents. In {\sl Proceedings of IEEE First Annual Workshop on Mobile and Ad hoc Networking and Computing}, IEEE, Piscataway, USA, pp. 145-146,2000. (Published Conference Proceedings style)

\bibitem{bib5} O. Hryniewicz. An evaluation of the reliability of complex systems using shadowed sets and fuzzy lifetime data. {\sl International Journal of Automation and Computing}, to be published.

\bibitem{bib6} W. Zhang. Reinforcement Learning for Job-shop Scheduling, Ph. D. dissertation, Oregon State University, USA,1996. (Dissertation style)

\bibitem{bib7} IEEE Criteria for Class IE Electric Systems, IEEE Standard 308, 1969. (Standards style)

\bibitem{bib8} R. C. Reily, J. L. Mack. The Self-organization of Spatially Invariant Representations, Technical Report PDP. CNS.92.5, Department of Psychology, Mellon University, USA, 1993. (Report style)

\bibitem{bib9} J. P. Wilkinson. Nonlinear Resonant Circuit Devices, U.S. Patent 362412, July 1990. (Patent style)

\bibitem{bib10} J. Jones. {\sl Networks}, 2nd ed., [Online], Available: http://www.atm.com, May 10, 1991.

\bibitem{bib11} R. J. Vidmar. On the use of atmospheric plasmas as electromagnetic reflectors. {\sl IEEE Transactions on Plasma Science}, vol. 21, no. 3, pp. 945-999, [Online], Available: http://www.halcyon.com, July 20-25, 1999.



\end{thebibliography}


